FSD: Fast Self-Supervised Single RGB-D to Categorical 3D Objects

In this work, we address the challenging task of 3D object recognition without the reliance on real-world 3D labeled data. Our goal is to predict the 3D shape, size, and 6D pose of objects within a single RGB-D image, operating at the category level and eliminating the need for CAD models during inference. While existing self-supervised methods have made strides in this field, they often suffer from inefficiencies arising from non-end-to-end processing, reliance on separate models for different object categories, and slow surface extraction during the training of implicit reconstruction models; thus hindering both the speed and real-world applicability of the 3D recognition process. Our proposed method leverages a multi-stage training pipeline, designed to efficiently transfer synthetic performance to the real-world domain. This approach is achieved through a combination of 2D and 3D supervised losses during the synthetic domain training, followed by the incorporation of 2D supervised and 3D self-supervised losses on real-world data in two additional learning stages. By adopting this comprehensive strategy, our method successfully overcomes the aforementioned limitations and outperforms existing self-supervised 6D pose and size estimation baselines on the NOCS test-set with a 16.4% absolute improvement in mAP for 6D pose estimation while running in near real-time at 5 Hz.

==> figures/chapter_2/inference_time.tex <==
\renewcommand{\arraystretch}{1.0}

\begin{table}[htb!]
\scriptsize
    \centering
\resizebox{0.46\textwidth}{!}{%
\begin{tabular}{l c c   } \hline
    Method & &    Average inference time per image~$\downarrow$\\
    \hline
    SSC-6D~\cite{peng2022self} & &    1.99 seconds \\ 
    Ours & &    0.20 seconds \\
    \hline
\end{tabular}
}
    \caption{Comparison of inference times against other self-supervised methods on one NVIDIA A100 GPU.}
    \label{tab:inference_time}
\end{table}

==> figures/chapter_2/shape_extraction.tex <==
\renewcommand{\arraystretch}{1.0}

\begin{table}[htb!]
\scriptsize
    \centering
\resizebox{0.46\textwidth}{!}{%
\begin{tabular}{l c  } \hline
    Method &  Avg. shape extraction time~$\downarrow$\\
    \hline
    Deep-SDF~\cite{peng2022self} &   0.15 seconds  \\ 
    Octree sampling based SDF~\cite{Irshad2022ShAPOIR} & 0.11 seconds   \\
    Batched octree sampling based SDF (\textbf{Ours}) & 0.01 seconds  \\
    \hline
\end{tabular}
}
    \caption{Comparison of shape extraction speeds across methods. Resolution for DeepSDF is 64 and Level of Detail (LoD) for octree and batched octree methods is 6. Analysis performed on one NVIDIA A100 GPU.}
    \label{tab:shape_time}
\end{table}
\vspace{-1em}
